DeepCap: Monocular Human Performance Capture Using Weak Supervision

Human performance capture is a highly important computer vision problem with many applications in movie production and virtual/augmented reality. Many previous performance capture approaches either required expensive multi-view setups or did not recover dense space-time coherent geometry with frame-to-frame correspondences. We propose a novel deep learning approach for monocular dense human performance capture. Our method is trained in a weakly supervised manner based on multi-view supervision completely removing the need for training data with 3D ground truth annotations. The network architecture is based on two separate networks that disentangle the task into a pose estimation and a non-rigid surface deformation step. Extensive qualitative and quantitative evaluations show that our approach outperforms the state of the art in terms of quality and robustness.

==> sec/discussion.tex <==
\section{Discussion an}
%
\label{sec:discussion}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par \textit{Unseen Poses.}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par \textit{Person-specific.}
%

==> sec/intro_old.tex <==
%
\section{Introduction}
%
\label{sec:intro}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par
%
Human performance capture revolutionized the film and gaming industry in the recent decades.
%
Apart from visual effects and computer animation applications, it also has vast use cases in generating personalized dynamic virtual avatars for telepresence, virtual try-on, and many other areas.
%
The majority of established systems can only capture sparse articulated motion (facial expression at most), while the tracking of dense full-body deformations of skin and clothing, which play an important role in producing realistic virtual characters, is still missing. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par
%
In the literature of dense full-body performance capture, multi-view marker-less methods \cite{bray06,brox06,brox10,cagniart10,de08,gall09,liu11,mustafa15,vlasic08,vlasic09, wu13,pons17,pons15} have shown compelling results. 
%
However, these approaches rely on well-controlled multi-camera studios (typically with green screen), which prohibits them from being used for location shootings of films and telepresence in living/working spaces. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
	%
	\begin{center}
		%
		\includegraphics[width=\linewidth]{images/teaser.png}
		%
	\end{center}
	%
	\caption
	{
		%
		We present the first learning-based approach for dense monocular human performance capture using weak multi-view supervision that not only predicts the pose but also the non-rigid deformations of the model surface.
		%
	}
	%
	\label{fig:teaser}
	%	
\end{figure}
%
\par
%
%Something like: alldieck, Bhatnagar reconstructs static clothing but not motion, PiFU and deep human are not models, that means they do not recover the skeletal structure, can not edit etc
%we are the first to learn non-rgid motion capture
%including skeleton and non-rigid layer 
%in a fully unsupervised manner
\GPM{Note that I focus intro on learning based methods, and therefore I discuss Habermann and Xu et al later}

Using a single RGB camera, recent learning based methods have shown compelling dense reconstruction of humans, including clothing, hair and facial details~\cite{saito19,zheng19,alldieck19,alldieck18a,bhatnagar2019mgn}.
One line of work directly regress voxels~\cite{zheng19} or the continuous occupancy of the surface~\cite{saito19}. Since predictions are pixel aligned reconstructions have nice detail, but the limbs of the person are often missing, specially for difficult poses. More importantly, the recovered motion is not factorized into articulation and non-rigid deformation, which do not permit control over the reconstructions, for example changing the pose or retarget of motion to novel characters \GPM{do we have this? would be cool}.  Furthermore, surface vertices are not tracked over time. Another line of work predict deformations or displacements to an articulated template, which prevents missing limbs and allows more control~\cite{alldieck19,bhatnagar2019mgn,alldieck2019tex2shape}.  However, these works assume clothing~\cite{alldieck19,bhatnagar2019mgn,alldieck2019tex2shape} does not change with pose and motion -- that is they do not capture motion and pose dependent deformations. 

What appears to be missing is a learning based model capable of jointly predicting 3D articulation and non-rigid motion, which naturally occurs when we move.  
In this paper, we propose a CNN model which integrates a fully differentiable \emph{mesh} template parameterized with \emph{pose} and an \emph{embedded deformation node graph}. 
%
While this parameterization has been used for model fitting~\cite{xu18,habermann19,yu18}, there exists no learning based method capable of inferring its parameters in a single feed-forward pass. 
\GPM{Still sounds weak, we need to distinguish us more from model-based methods}
%
From a single image, our network predicts the skeletal pose, and the rotation and translation parameters for each node in the deformation graph. In stark contrast to previous implicit function based representations~\cite{saito19, zheng19}, our mesh-based method \emph{tracks the surface vertices over time}, which is crucial for mesh compression, for adding semantics, and for texturing the surface. Furthermore, by virtue of our paremeterization, our model always produces a human surface \emph{without missing limbs}, even during occlusions and out of plane motions. 

While previous methods~\cite{saito19,zheng19,alldieck19,bhatnagar2019mgn} rely on 3D scans for training, our method is self-supervised directly from multi-view images.
%To eliminate the need for generating ground truth annotation, we propose a weakly supervised approach for monocular human performance capture, which reconstructs the dense non-rigid surface deformation of the human body in general clothing using just a single RGB camera.
%
To this end, we propose a fully differentiable network which is trained in an analysis-by-synthesis fashion, without explicitly using any 3D ground truth annotation.
%
%
Specifically, during training, our method only requires a personalized template mesh of the actor and a multi-view video sequence of the actor performing various motions -- our network learns by comparing its single image feed-forward predictions against the multi-view 2D observations.
%
From a single image, our network predicts the deformed template, and compares its rendering against 
the corresponding multi-view 2D images in a differentiable manner, effectively learning from video footage directly.
%renders it in a differentiable way and computes a 2D loss by comparing the rendering with the multi-view 2D observations.
%
To regularize this heavily underconstrained problem, we found that training the pose and the non-rigid part in stages improves stability. 
%
%
%In our network architecture, we propose a differentiable deformation representation of the template that combines skinning and embedded deformation.
%
%This enables us to disentangle pose from non-rigid deformations and tackle these two sub-problems separately.
%
%The training of our method consists of two stages:
%
%First, we train a pose prediction network to regress the 3D pose of the actor in the form of joint angles and the camera relative rotation.
%
%After that, our second network regresses the non-rigid deformation of the surface that cannot be modeled by the skeletal pose.
%
%Instead of using ground truth supervision, our method renders the deformed template in a differentiable way and computes the loss by comparing the rendering with the multi-view 2D observations.
%
At test time, our method only requires a single-view image as input and produces a deformed template matching the actor's non-rigid motion in the image.
%
In summary, the main technical contributions of our work are:
%
\begin{itemize}
	%
	\item{A learning-based 3D human performance capture approach that jointly tracks the skeletal pose and the non-rigid surface deformations from monocular images.}
	%
	\item{A new differentiable representation of deforming human surfaces which enables training from multi-view video footage directly.}
	%
\end{itemize}
%
Our new model achieves high quality dense human performance results on our new dataset, demonstrating, qualitatively and quantitatively, the advantages of our approach over previous methods on various challenging scenarios.
\GPM{no mention of real time?}
%This enables us to disentangle pose from non-rigid deformations and tackle these two sub-problems separately.
%Recently, there have been incessant attempt in democratizing human performance capture by using a single RGB camera \cite{xu18,habermann19,saito19,zheng19}.
%
%Most of these methods leverage deep neural networks (DNNs) to tackle the challenging monocular reconstruction problem, which is ill-posed due to the inherent depth ambiguity of the single view setting.
%
%Unsurprisingly, these methods rely on large scale training datasets with ground truth annotation -- either sparse 3D joint positions \cite{xu18,habermann19}, or dense 3D shapes \cite{saito19,zheng19}.
%
%However, obtaining the 3D annotations at large scale is not only challenging, but also time-consuming and expensive.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par
%

%
